From Coarse to Fine: Robust Hierarchical Localization at Large Scale

Robust and accurate visual localization is a fundamental capability for numerous applications, such as autonomous driving, mobile robotics, or augmented reality. It remains, however, a challenging task, particularly for large-scale environments and in presence of significant appearance changes. State-of-the-art methods not only struggle with such scenarios, but are often too resource intensive for certain real-time applications. In this paper we propose HF-Net, a hierarchical localization approach based on a monolithic CNN that simultaneously predicts local features and global descriptors for accurate 6-DoF localization. We exploit the coarse-to-fine localization paradigm: we first perform a global retrieval to obtain location hypotheses and only later match local features within those candidate places. This hierarchical approach incurs significant runtime savings and makes our system suitable for real-time operation. By leveraging learned descriptors, our method achieves remarkable localization robustness across large variations of appearance and sets a new state-of-the-art on two challenging benchmarks for large-scale localization.

==> tables/timings_old.tex <==
\setlength\tabcolsep{3.0pt}
\begin{tabular}{ll|c|c|c|c|c|c||c|c|c||c|c|c|c}&& \multicolumn{6}{c||}{\textbf{HF-Net (ours)}}& \multicolumn{3}{c||}{\textbf{AS}}&
\multicolumn{4}{c}{\textbf{NV+SIFT}}\\
&& {HF-Net}& {Global search}& {Covisibility}& {Local search}& {PnP+RANSAC}& {\textbf{Total}}& {SIFT}& {Loc.}& {\textbf{Total}}& {SIFT}& {NetVLAD}& {Loc.}& {\textbf{Total}}\\ \cline{3-15}
\multirow{2}{*}{Aachen} & Day & 15 & 51 & 5 & 163 & 9 & \textbf{243} & 263 & 112 & \textbf{375} & 263 & 92 & 1264 & \textbf{1356}\\ \cline{3-15}
& Night & 15 & 52 & 5 & 170 & 18 & \textbf{260} & 263 & 132 & \textbf{395} & 263 & 92 & 1563 & \textbf{1655}\\ \hline
\multirow{2}{*}{RobotCar} & Dusk & 19 & 53 & 1 & 58 & 4 & \textbf{135} & 189 & 283 & \textbf{472} & 189 & 91 & 294 & \textbf{385} \\ \cline{3-15}
& Night & 19 & 55 & 1 & 103 & 38 & \textbf{216} & 189 & 1021 & \textbf{1210} & 189 & 91 & 554 & \textbf{645}\\ \hline
\end{tabular}
